Multiplicative Error Models: 20 years on

Several phenomena are available representing market activity: volumes, number of trades, durations between trades or quotes, volatility - however measured - all share the feature to be represented as positive valued time series. When modeled, persistence in their behavior and reaction to new information suggested to adopt an autoregressive-type framework. The Multiplicative Error Model (MEM) is borne of an extension of the popular GARCH approach for modeling and forecasting conditional volatility of asset returns. It is obtained by multiplicatively combining the conditional expectation of a process (deterministically dependent upon an information set at a previous time period) with a random disturbance representing unpredictable news: MEMs have proved to parsimoniously achieve their task of producing good performing forecasts. In this paper we discuss various aspects of model specification and inference both for the univariate and the multivariate case. The applications are illustrative examples of how the presence of a slow moving low-frequency component can improve the properties of the estimated models.

==> Table/Tab-spmem-gof-01.tex <==
\scalebox{1}{
\begin{tabular}{rrrrrrrrrr}
  & DJI & IXIC & SPX & FCHI & GDAXI & STOXX50E & HSI & KS11 & N225 \\ 
  \hline
Anderson-Darling.gamma         & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\ 
  Anderson-Darling.lognormal   & 0.0764 & 0.0270 & 0.1278 & 0.0081 & 0.0005 & 0.0000 & 0.0000 & 0.0185 & 0.0000 \\ 
  Anderson-Darling.betaprime   & 0.1055 & 0.0369 & 0.2194 & 0.0184 & 0.0011 & 0.0000 & 0.0000 & 0.0325 & 0.0000 \\ 
  Anderson-Darling.loglogistic & 0.0496 & 0.0705 & 0.0000 & 0.0000 & 0.0218 & 0.4204 & 0.1194 & 0.0513 & 0.0524 \\ 
  Cramer-VonMises.gamma        & 0.0004 & 0.0001 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0008 & 0.0000 \\ 
  Cramer-VonMises.lognormal    & 0.1578 & 0.0482 & 0.1650 & 0.0237 & 0.0034 & 0.0001 & 0.0002 & 0.0430 & 0.0000 \\ 
  Cramer-VonMises.betaprime    & 0.2082 & 0.0628 & 0.2486 & 0.0450 & 0.0059 & 0.0002 & 0.0005 & 0.0699 & 0.0000 \\ 
  Cramer-VonMises.loglogistic  & 0.0708 & 0.0883 & 0.0001 & 0.0007 & 0.0340 & 0.7570 & 0.1034 & 0.0833 & 0.0580 \\ 
   \hline
\end{tabular}
}


==> Table/Tab-spvmem-gof-01.tex <==
\scalebox{1}{
\begin{tabular}{rrrrrrrrrr}
  & DJI & IXIC & SPX & FCHI & GDAXI & STOXX50E & HSI & KS11 & N225 \\ 
  \hline
  Anderson.Darling.gamma         & 0.0000 & 0.0835 & 0.0000 & 0.0000 & 0.0000 & 0.0117 & 0.0000 & 0.0000 & 0.0001 \\ 
  Anderson.Darling.lognormal     & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\ 
  Anderson.Darling.betaprime     & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\ 
  Anderson.Darling.loglogistic   & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\ 
  Cramer.VonMises.gamma          & 0.0077 & 0.1368 & 0.0000 & 0.0000 & 0.0009 & 0.0120 & 0.0001 & 0.0356 & 0.0196 \\ 
  Cramer.VonMises.lognormal      & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\ 
  Cramer.VonMises.betaprime      & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\ 
  Cramer.VonMises.loglogistic    & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\ 
  Anderson.Darling.gamma.1       & 0.0003 & 0.0001 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0043 & 0.0000 \\ 
  Anderson.Darling.lognormal.1   & 0.3403 & 0.1577 & 0.4096 & 0.0113 & 0.0038 & 0.0001 & 0.0052 & 0.1816 & 0.0000 \\ 
  Anderson.Darling.betaprime.1   & 0.4102 & 0.1964 & 0.6147 & 0.0248 & 0.0074 & 0.0003 & 0.0106 & 0.2603 & 0.0000 \\ 
  Anderson.Darling.loglogistic.1 & 0.0123 & 0.0204 & 0.0000 & 0.0000 & 0.0132 & 0.4805 & 0.0066 & 0.0066 & 0.0240 \\ 
  Cramer.VonMises.gamma.1        & 0.0033 & 0.0010 & 0.0005 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0170 & 0.0000 \\ 
  Cramer.VonMises.lognormal.1    & 0.4764 & 0.2425 & 0.3540 & 0.0315 & 0.0137 & 0.0010 & 0.0204 & 0.2419 & 0.0000 \\ 
  Cramer.VonMises.betaprime.1    & 0.5704 & 0.2878 & 0.5225 & 0.0583 & 0.0235 & 0.0022 & 0.0353 & 0.3227 & 0.0001 \\ 
  Cramer.VonMises.loglogistic.1  & 0.0260 & 0.0286 & 0.0000 & 0.0007 & 0.0243 & 0.6014 & 0.0099 & 0.0218 & 0.0267 \\ 
  Anderson.Darling.gamma.2       & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\ 
  Anderson.Darling.lognormal.2   & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\ 
  Anderson.Darling.betaprime.2   & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\ 
  Anderson.Darling.loglogistic.2 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\ 
  Cramer.VonMises.gamma.2        & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\ 
  Cramer.VonMises.lognormal.2    & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\ 
  Cramer.VonMises.betaprime.2    & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\ 
  Cramer.VonMises.loglogistic.2  & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\ 
   \hline
\end{tabular}
}


==> Table/Tab-vmem-heavy-01.tex <==
\scalebox{1}{
\begin{tabular}{rrrrrrrrrr}
  & DJI & IXIC & SPX & FCHI & GDAXI & STOXX50E & HSI & KS11 & N225 \\ 
  \hline
stat & 12.3104 & 25.1204 & 51.7463 & 61.3916 & 39.4824 & 31.1643 & 28.7689 & 23.0047 & 42.0453 \\ 
  pval & 0.0064 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\ 
  stat.1 & 16.1555 & 32.5538 & 83.4393 & 57.5994 & 76.6602 & 46.0709 & 56.6530 & 31.1979 & 87.8567 \\ 
  pval.1 & 0.0011 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\ 
   \hline
\end{tabular}
}

